Deeply Coupled Cross-Modal Prompt Learning

Recent advancements in multimodal foundation models (e.g., CLIP) have excelled in zero-shot generalization. Prompt tuning involved in the knowledge transfer from foundation models to downstream tasks has gained significant attention recently. Existing prompt-tuning methods in cross-modal learning, however, either solely focus on language branch, or learn vision-language interaction in a shallow mechanism. In this context, we propose a Deeply coupled Cross-modal Prompt learning (DCP) method based on CLIP. DCP flexibly accommodates the interplay between vision and language with a Cross-Modal Prompt Attention (CMPA) mechanism, which enables the mutual exchange of respective representation through a well-connected multi-head attention module progressively and strongly. We then conduct comprehensive few-shot learning experiments on 11 image classification datasets and analyze the robustness to domain shift as well. Thorough experimental analysis evidently demonstrates the superb few-shot generalization and compelling domain adaption capacity of a well-executed DCP. The code can be found at https://github.com/GingL/CMPA.

==> cons.tex <==


\section{Discussion and Conclusion}
Recent advancements in pre-trained large foundation models, such as CLIP, have demonstrated exceptional performance in zero-shot learning. Prompt tuning, which efficiently leverages the general knowledge from these models to improve the performance of downstream tasks, has gained significant attention. However, previous prompt-tuning methods either solely focus on language branch, or learn the interaction between vision and language in a shallow mechanism. In this paper, we propose a \textbf{D}eeply coupled \textbf{C}ross-modal \textbf{P}rompt learning (DCP) method based on CLIP. DCP learns the correspondence between vision and language with a \textbf{C}ross-\textbf{M}odal \textbf{P}rompt \textbf{A}ttention (CMPA) mechanism. The CMPA enhances the interaction between vision and language through a cross-modal multi-head attention. With such design, the text encoder can learn the text embedding under the guidance of image information and vice versa. DCP is an efficient and effective way to strengthen communication between visual and text with only a small number of trainable parameters, which combines the advantages of dual-branch and single branch multi-modal pre-training methods. We conduct experiments on 11 image classification datasets in few-shot settings. Comprehensive experimental analysis demonstrates that DCP that operates on both language and vision modality in a deep manner, is a superior method for few-shot learning, which is evidenced by its top performance.

\section{Limitations}
% 类别数目多的数据集，shot数越少的情况下，epoch越多性能越差，如sun397和imagenet
There is a strange phenomenon in our experiments and we have not yet found the cause. For datasets with a large number of categories, the lower the number of shots, the worse the performance with more epochs, such as Sun397 and ImageNet.

==> experiments.tex <==
\section{Experiments}

\begin{figure*}[tp]
\centering
\includegraphics[width=\textwidth]{figs/fewshot_results.pdf}
\caption{\textbf{Main results of few-shot image classification on 11 datasets.} The accuracy (\%) is the average over three runs on 1/2/4/8/16 shots. Overall, our DCP ({\color{red} red line}) outperforms other methods by a large margin on the average results of 11 datasets.}
\label{fig:fewshot_results}
\end{figure*}
In this section, we conduct experiments to evaluate the effectiveness of our method under two settings. One is few-shot visual recognition including 11 different datasets covering generic objects, scenes, actions and fine-grained categories. The other is domain adaptation test, where we train our model in ImageNet and evaluate on other four datasets.

\subsection{Few-shot Learning}
% 数据集
\subsubsection{Datasets}
Following CoOp~\cite{DBLP:conf/emnlp/LesterAC21}, we evaluate our method on 11 public visual recognition datasets: ImageNet~\cite{DBLP:conf/cvpr/DengDSLL009}, Caltech101~\cite{DBLP:conf/cvpr/LiFP04}, OxfordPets~\cite{DBLP:conf/cvpr/ParkhiVZJ12}, StanfordCars~\cite{DBLP:conf/iccvw/Krause0DF13}, Flowers102~\cite{DBLP:conf/icvgip/NilsbackZ08}, Food101~\cite{DBLP:conf/eccv/BossardGG14}, FGVCAircraft~\cite{DBLP:journals/corr/MajiRKBV13}, SUN397~\cite{DBLP:conf/cvpr/XiaoHEOT10}, DTD~\cite{DBLP:conf/cvpr/CimpoiMKMV14}, EuroSAT~\cite{DBLP:journals/staeors/HelberBDB19} and UCF101~\cite{DBLP:journals/corr/abs-1212-0402}. 
We also use the same 1, 2, 4, 8, 16 shots as CoOp for training and the full test set for testing. The reported results are the average over three runs with different random seeds. 


% 训练设置
\subsubsection{Implementation Details}
We use the pre-trained ViT-B/16 CLIP model as our backbone. The length of prompt tokens for visual and text are both defined as 16. The prompt length is 9 as a trade-off between accuracy and training efficiency. We set the batch-size to 4 with a learning rate of 0.0035 via SGD optimizer. We use 20 epochs for most datasets, except ImageNet, SUN397 and Food101. For Food101, 5 epochs is used for all shots. We use 5 epoch for 1, 2 and 4 shots on ImageNet, and 1, 2 shots on SUN397. 

% 整体11个数据集结果
\subsubsection{Main Results}
% \begin{figure*}[tp]
% 	\centering
% 		\subcaptionbox{}{	
% 		\includegraphics[width=0.3\textwidth]{figs/fewshot_plot/imagenet.png}}
% 	\hfill
% 	\subcaptionbox{}{
% 		\includegraphics[width=0.3\textwidth]{figs/fewshot_plot/imagenet.png}}
% 	\hfill
% 	\subcaptionbox{}{
% 		\includegraphics[width=0.3\textwidth]{figs/fewshot_plot/caltech101.png}}
  
	% \subcaptionbox{}{
	% 	\includegraphics[width=0.33\textwidth]{figs/fewshot_plot/oxford_pets.png}}
 %  	\hfill
	% \subcaptionbox{}{
	% 	\includegraphics[width=0.33\textwidth]{figs/fewshot_plot/stanford_cars.png}
	% \hfill
	% \subcaptionbox{}{
	% 	\includegraphics[width=0.33\textwidth]{figs/fewshot_plot/oxford_flowers.png}

	% \subcaptionbox{}{
	% 	\includegraphics[width=0.33\textwidth]{figs/fewshot_plot/food101.png}}
 %  	\hfill
	% \subcaptionbox{}{
	% 	\includegraphics[width=0.33\textwidth]{figs/fewshot_plot/fgvc_aircraft.png}
 %  	\hfill
	% \subcaptionbox{}{
	% 	\includegraphics[width=0.33\textwidth]{figs/fewshot_plot/sun397.png}

	% \subcaptionbox{}{
	% 	\includegraphics[width=0.33\textwidth]{figs/fewshot_plot/dtd.png}
 %  	\hfill
	% \subcaptionbox{}{
	% 	\includegraphics[width=0.33\textwidth]{figs/fewshot_plot/eurosat.png}}
 %  	\hfill
	% \subcaptionbox{}{
	% 	\includegraphics[width=0.33\textwidth]{figs/fewshot_plot/ucf101.png}}
% 	\caption{}
% 	\label{fig:}
% \end{figure*}

\paragraph{Compared Methods.}
We compare our method with the original zero-shot CLIP, text prompt learning (CoOp), visual prompt learning (VPT) and multi-modal prompt learning (MaPle). All these methods use ViT-B/16 as backbone. We follows the implementation of MaPle~\cite{DBLP:journals/corr/abs-2210-03117}. The prompt length of CoOp is set to 16. 
VPT uses a prompt length of 8 and the visual and text prompt length of MaPle is 2. The training epoch of CoOp is defined as 10, and that of VPT and MaPle is 5. 
We use the deep variant of VPT in few-shot experiments.
The prompt depth of MaPle is 9 as their original setting.  

% 细节结果分析
\paragraph{Performance Analysis.}
% 整体来说，shot数越高，我们的方法越好
Figure~\ref{fig:fewshot_results} demonstrates our results comparison with other methods. The top left sub-figure shows the average performance of four methods. We can have the following findings. 
1) Cross-modal prompt learning (DCP, MaPle) gets a large performance gain compared with single-modal prompt learning methods (VPT, CoOp). VPT and CoOp achieves comparable performance on different shots. These results demonstrate the superiority of cross-modal prompt learning over uni-modal prompt learning.
2) Although both belong to multi-modal prompt learning methods, our method still outperforms MaPle on 1/2/4/8/16 shots settings by 1.72/3.18/3.19/2.20/2.76(\%). MaPle utilized a linear layer to generates visual prompts from text prompts. Our proposed DCP enhances the interaction between vision and language with a cross-modal prompt attention, which can not only guide visual embedding learning through text prompts, but also influence the language embedding with visual prompts. 
3) Compared with 2/4/8/16 shots, our approach achieves a lower performance gain on 1 shot. We can also find that on separate datasets, our method achieves the best performance in almost all 16-shot cases (except Food101).
This phenomenon indicates that our method is more effective in cases where the number of shots is relatively large. This is perhaps because the alignment between different modals is more challenging due to the small number of samples per category.

% 我们的方法在flower 102， stanford cars，fgvc和euroset上结果提升显著，说明我们的方法可能更适合这种细粒度的分类
For individual datasets, we find that our approach has significant performance improvements on Flowers102, StanfordCars, FGVCAircraft, and EuroSAT. However, on 
the datasets of general category such as ImageNet and Caltech101, our method does not achieve satisfactory performance when the number of shots is less than 16. We can conclude that our method is more robust for fine-grained classification datasets, and we need more shots for general category classification.
%在food101上表现不好，而且在food101上所有方法的1shot都无法超越zero shot，可能是food101本身的few-shot的数目不够cover test集的表现，分布理论，通过mmd浅算一下. Noisy training data.
On the dataset of Food101, our method performs slightly lower than maple. We also find that all methods underperform zero-shot on 1-shot setting. 
We suppose this phenomenon comes from the noisy training data of Food101~\cite{DBLP:conf/eccv/BossardGG14}, which may cause the overall relationship between $D_{fss} + D_{pre-train}$ and $D_{test}$ deteriorates as compared to that of $D_{pre-train}$ and $D_{test}$ or $distance(D_{fss} + D_{pre-train}, D_{test} > distance(D_{pre-train}, D_{test})$, where $D_{pre-train}$ is the image-text set for pre-training, $D_{fss}$ is the few-shot set and $D_{test}$ is the distribution of the test set.

% ablation study 1. 长度， 宽度， 不同融合方式， 参数是否共享
\subsubsection{Ablation Study}
% \paragraph{Prompt Depth.}
The are two important settings in CMPA: the feature fusion method in different prompts and parameter sharing of CMPA across different layers. We conduct corresponding ablation experiments in this section to find the optimal setting.
\paragraph{Feature Fusion in Prompts.}
% there is a plot
\begin{figure}[tp]
	\centering
	\includegraphics[width=0.48\textwidth]{figs/fewshot_plot/all.png}
	\caption{The comparison of different feature fusion methods.}
	\label{fig:feat_fuse}
\end{figure}
Before the visual and text prompts are fed into the CMPA, the dimension of the batchsize should be consistent. The defined batchsize only affects visual prompt while the batchsize of text prompts actually the number of the dataset due to the implementation of CLIP. We conduct three settings to align the batchsize of visual and text prompts. The result comparison is shown in Figure~\ref{fig:feat_fuse}. 
`avg' means that we use the average of of visual and text prompts across the dimension of batch.
`max' stands for using the features with highest response across the batch dimension as the visual and text prompts. 
`first' represents that we select the first embedding across the batch dimension of visual and text prompts to feed into CMPA.

\paragraph{Parameter Sharing.}
\begin{table}[]
\begin{tabular}{cccccc}
\toprule
PS & 2& 4& 6& 8& 16      \\ \midrule
True& 68.99   & 72.56   & 75.69   & 78.42   & 80.55   \\
False& 67.42   & 71.34   & 75.27   & 78.49   & 80.53   \\ \bottomrule
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}
\end{tabular}
\caption{Parameter Sharing}
\label{tab:ps}
\end{table}
We intend to learn as few parameters as possible to achieve a transfer of large-scale pre-trained models in downstream tasks. Setting the prompt depth to 9 means that there are 9 CMPA modules, which greatly increases the number of trainable parameters for the model. Hence we conduct experiment in which the parameters of CMPA are shared across different layer. Table~\ref{tab:ps} shows the average results of different shots on 11 datasets. `PS' is short for `parameter sharing'. `True' and `False' denote whether to use parameter sharing or not. It can be observed that on most shots (except 8 shot) the performance of parameter sharing is higher than non-sharing setting. 

\begin{table*}[]
\centering
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{Method} & Source         & \multicolumn{4}{c}{Target}  & \multirow{2}{*}{Average} & \multirow{2}{*}{OOD Average} \\ \cline{2-6}
& ImageNet& -V2     & -S & -A     & -R     &&    \\ \midrule
CLIP& 66.73   & 60.83   & 46.15& 47.77   & 73.96   & 59.09& 57.18\\ \midrule
CoOp& 71.53   & 64.20   & 47.99& 49.71   & 75.21   & 61.73& 59.28\\
CoCoOp     & 71.02   & 64.07   & 48.75& 50.63   & 76.18   & 62.13& 59.91\\
VPT-Deep   & 70.57   & 63.67   & 47.66& 43.85   & 74.42   & 60.03& 57.40\\ \midrule
MaPle      & 71.02   & 64.07   & \textbf{49.15}  & \textbf{50.90} & \textbf{76.98} & \redfont{62.42}& \textbf{60.28}  \\
UPT & \textbf{72.63} & \redfont{64.35}   & 48.66& \redfont{50.66}   & 76.24   & \textbf{62.51}& \redfont{59.98}\\ \midrule
DCP (ours) & \redfont{71.53}   & \textbf{64.50} & \redfont{48.77}& 49.40   & \redfont{76.50}   & 62.14& 59.79 \\ \bottomrule  
\end{tabular}
\caption{}
\label{tab:xd}
\end{table*}
% 跨域实验
\subsection{Domain Generalization}
After prompt tuning on specific datasets, we do not want to lose the general knowledge of the pre-trained large model.  In this section, we conduct domain adaptation tests to evaluate the generalization ability of our model DCP. 
%数据集
\subsubsection{Datasets and Implementation Details}
Following \cite{DBLP:journals/ijcv/ZhouYLL22}, we use ImageNet~\cite{DBLP:conf/cvpr/DengDSLL009} as source domain, and ImageNet V2~\cite{DBLP:conf/icml/RechtRSS19}, ImageNet-Sketch~\cite{DBLP:conf/nips/WangGLX19}, ImageNet-A~\cite{DBLP:conf/cvpr/HendrycksZBSS21} and ImageNet-R~\cite{DBLP:conf/iccv/HendrycksBMKWDD21} as target domain. We train our model on the 16 shot of ImageNet, and test it on other four datasets.
%训练设置
Different from the settings in few-shot task, the training epoch on 16-shot ImageNet in cross domian task is set to 5. We also decrease the prompt length as 8.
% 整体结果
\subsubsection{Main Results}
Table~\ref{tab:xd} compares our method DCP with prompt learning methods on cross domain tasks.
The compared methods include zero-shot CLIP, unimodal prompt learning methods (CoOp, CoCoOp and VPT-Deep) and multi-modal prompt learning methods (Maple and UPT).
The best results on different datasets are in bold, and the second best results are in red. We can observe that 
1) prompt learning does not corrupt the generalization ability of pre-trained large models;
2) multi-modal prompt learning methods outperform unimodal prompt learning methods in generalization performance;
3) our method can get comparable performance as the state-of-the-art method.



==> intro.tex <==
\section{Introduction}
% 预训练模型的发展和优势，general knowledge transfer
Large foundation models pre-trained on millions of image-text pairs such as CLIP~\cite{DBLP:conf/icml/RadfordKHRGASAM21} and ALIGN~\cite{DBLP:conf/icml/JiaYXCPPLSLD21} have shown promising performance on zero-shot image classification. Research has repeatedly shown that the general knowledge learned by the foundation models are also transferred to various downstream tasks, such as few-shot image classification~\cite{DBLP:journals/ijcv/ZhouYLL22,DBLP:conf/cvpr/ZhouYL022}, visual grounding~\cite{DBLP:conf/acl/SubramanianMD0022}, visual question answering~\cite{DBLP:conf/ijcai/Liu0P022} and so on. The utilization of these methods exhibits a significant potential in open-vocabulary scenarios. Thus, the challenge associated with how to efficiently and effectively adapt large pre-trained models to downstream tasks has garnered increasing attention especially in low-resources training scenarios.


% 当前对clip的应用无法通过fine-tune，prompt tune这种方式很efficient，列举现有的prompt tuning的方法，然后现有的这些prompt learning method每一层都是随机生成初始化的，与前一层无关，这一点也是让人无法理解的
Directly fine-tuning the foundation model is infeasible due to the massive training parameters and the catastrophic forgetting caused by overfitting~\cite{DBLP:journals/corr/KirkpatrickPRVD16}. 
In contrast, the parameter-efficient \emph{prompt tuning} approach explored in natural language processing has yielded significant success~\cite{DBLP:conf/emnlp/LesterAC21}, leading to an increased examination of this technique within the realm of multi-modality, especially in the language-branch of CLIP.
For example,
CoOp~\cite{DBLP:journals/ijcv/ZhouYLL22} and ProDA~\cite{DBLP:conf/cvpr/LuLZL022} explore the vanilla few-shot learning based on CLIP by adjusting the embedding or distribution of the text prompt. 
CoCoOp~\cite{DBLP:conf/cvpr/ZhouYL022} and ProGrad~\cite{DBLP:journals/corr/abs-2205-14865} focus more on the unseen classes. They update the text prompt either with the supervision of image information or tweak gradient direction to improve the generalization ability of the model.

The above approaches only adjust the text embedding of CLIP and neglect the visual branch. The success of VPT~\cite{DBLP:conf/eccv/JiaTCCBHL22} demonstrates the effectiveness of visual prompt learning. Inspired by this work, UPT~\cite{DBLP:journals/corr/abs-2210-07225} and MaPLe~\cite{DBLP:journals/corr/abs-2210-03117} simultaneously tune the visual and text prompts. 
UPT improves the few-shot learning ability by generating the visual and text prompts. MaPLe achieves better performance in the classification of unseen classes. 
These methods uncover the underlying rationale and limitations of dual-branch prompt tuning.

% 但是clip这种dual encoder的结构只通过contrastive learning去学习两种模态的对齐，对于视觉和语言之间的交互学习是不足的。因此，一方面为了能够利用clip的general knowledge，另一方面为了高效地实现视觉语言之间的交互，我们提出了CMPA
Specifically, the dual-branch CLIP learn the visual and language correspondence only based on contrastive learning, where vision and language branches lack mutual communication at the early stage of the network. Multi-modal prompt learning techniques, such as MaPLe and UPT, incorporate language-vision interactions of the network and achieve significantly improved performance, highlighting the significance of the interactions between language and vision. However, previous studies have leveraged language-vision interactions at a superficial level. For example, UPT generate visual and text prompts before they are fed into the corresponding encoder. MaPLe only utilize language prompt to generate visual prompts. 
Many work~\cite{DBLP:conf/iclr/DosovitskiyB0WZ21,DBLP:conf/icml/WangYMLBLMZZY22} has shown that neural networks, especially transformer-based models, can leverage the deep fusion of information from multiple views to improve their performance, an aspect that has not been fully explored in the field of multi-modality few-shot learning. To this end, we design \textbf{D}eeply coupled \textbf{C}ross-modal \textbf{P}rompt learning (DCP) enhancing the language-vision interaction. Specifically, DCP is built based on CLIP, with additional text and visual prompts across multiple layers. 
Different from previous methods with deep prompt tuning~\cite{DBLP:conf/eccv/JiaTCCBHL22,DBLP:journals/corr/abs-2210-07225,DBLP:journals/corr/abs-2210-03117}, DCP only initializes the first layer of visual and text prompt with random vectors. The following prompts are generated by \textbf{C}ross-\textbf{M}odal \textbf{P}rompt \textbf{A}ttention (CMPA) module, which combines the prompts from the previous layer of two modalities. CMPA brings stronger connection from two aspects, that is, \emph{Depth} and \emph{Breadth}. 1) \emph{Depth} means that CMPA strengthens the correlation of the prompts among different layers. 2) \emph{Breadth} suggests that CMPA enhances the interaction between visual and language modalities. CMPA is the core module to realize the deeply couple between two modalities.
DCP with CMPA actually combines the advantages of single branch and dual-branch multi-modal pre-training methods, which can decrease the discrepancy between visual and text knowledge without adding too much trainable parameters.

% CMPA是一种怎样的方法，有哪些优势
To conclude, the contributions of this work are as follows:
\begin{itemize}
    \item We design a deeply coupled cross-modal prompt learning (DCP) method with a core module cross-modal prompt attention (CMPA). CMPA can enhance the interaction between visual and language modals as well as different layers. 
    \item We verify our method on 11 datasets covering different image classification tasks including generic objects, scenes, actions and fine-grained categories. Our method outperforms visual prompt tuning, text prompt tuning and multi-modal prompt tuning methods under few-shot setting.
    \item We conduct experiments on domain adaptation tasks. Our method achieves comparable performance of the state-of-the-art methods, indicating the robustness of our method. 
\end{itemize}


% Large foundation models pre-trained on millions of image-text pairs such as CLIP~\cite{DBLP:conf/icml/RadfordKHRGASAM21} and ALIGN~\cite{DBLP:conf/icml/JiaYXCPPLSLD21} have shown promising performance on zero-shot image classification. \jh{The}{Research has repeatedly shown that the} general knowledge learned by the foundation models are also transferred to various downstream tasks, such as few-shot image classification~\cite{DBLP:journals/ijcv/ZhouYLL22,DBLP:conf/cvpr/ZhouYL022}, visual grounding~\cite{DBLP:conf/acl/SubramanianMD0022}, visual question answering~\cite{DBLP:conf/ijcai/Liu0P022} and so on. \jh{These methods show impressive potential in open-vocabulary scenarios. How to adapt the large foundation models to downstream tasks effectively and effectively attracts more attention.}{The utilization of these methods exhibits a significant potential in open-vocabulary scenarios. Thus, the challenge associated with how to efficiently and effectively adapt large pre-trained models to downstream tasks has garnered increasing attention especially in low-resources training scenarios.}


% % 当前对clip的应用无法通过fine-tune，prompt tune这种方式很efficient，列举现有的prompt tuning的方法，然后现有的这些prompt learning method每一层都是随机生成初始化的，与前一层无关，这一点也是让人无法理解的
% Directly fine-tuning the foundation model is infeasible due to the massive training parameters and the catastrophic forgetting caused by overfitting \jhcomment{}{(citation here)}. 
% In contrast, \jh{the parameter-efficient prompt tuning has achieved great success in natural language processing~\cite{DBLP:conf/emnlp/LesterAC21}}{the parameter-efficient \emph{prompt tuning} approach explored in natural language processing has yielded significant success~\cite{DBLP:conf/emnlp/LesterAC21}, leading to an increased examination of this technique within the realm of multi-modality, especially in the language-branch of CLIP.}
% \jh{As an efficient way to transfer general knowledge learned by large foundation model.}{}For example,
% CoOp~\cite{DBLP:journals/ijcv/ZhouYLL22} and ProDA~\cite{DBLP:conf/cvpr/LuLZL022} explore the vanilla few-shot learning based on CLIP by adjusting the embedding or distribution of the text prompt. 
% CoCoOp~\cite{DBLP:conf/cvpr/ZhouYL022} and ProGrad~\cite{DBLP:journals/corr/abs-2205-14865} focus more on the unseen classes. They update the text prompt either with \jh{image cooperation}{the supervision of image information} or \jh{changing}{tweak} gradient direction to improve the generalization ability of the model.

% The above approaches only adjust the text embedding of CLIP and neglect the visual branch. The success of VPT~\cite{DBLP:conf/eccv/JiaTCCBHL22} demonstrates the effectiveness of visual prompt learning. Inspired by this work, UPT~\cite{DBLP:journals/corr/abs-2210-07225} and MaPLe~\cite{DBLP:journals/corr/abs-2210-03117} simultaneously tune the visual and text prompts. UPT improves the few-shot learning ability by generating the visual and text prompts with a lightweight self-attention network. MaPLe achieves better performance in the classification of unseen classes by introducing the visual prompts \jh{learned from}{conditioned by} text prompts. \jhcomment{}{I think the description of UPT and MaPLe is a little duplicate with the next section, considering shorten or delete them.} These methods \jh{reveal the mask of dual-branch prompt tuning and realize promising performance}{uncover the underlying rationale and limitations of dual-branch prompt tuning}.

% % 但是clip这种dual encoder的结构只通过contrastive learning去学习两种模态的对齐，对于视觉和语言之间的交互学习是不足的。因此，一方面为了能够利用clip的general knowledge，另一方面为了高效地实现视觉语言之间的交互，我们提出了CMPA
% \jh{The}{Specifically, the} dual-branch CLIP learn the visual and language \jh{correspondence}{consistency} \st{only} based on contrastive learning, \jh{}{where vision and language branches lack mutual communication at the early stage of the network.} \jh{Although the multi-modal prompt learning could provide a certain interaction between visual and language, such interaction is still learned in a plain mechanism.}{Multi-modal prompt learning techniques, such as MaPLe and UPT, incorporate language-vision interactions at the early stages of the network and achieve significantly improved performance, highlighting the significance of the interactions between language and vision.} \jh{}{However, previous studies have leveraged language-vision interactions at a superficial level.} For example, UPT generate visual and text prompts before they are fed into the corresponding encoder. MaPLe only utilize language prompt to generate visual prompts. 
% \jh{}{Many work (find some citations here such as ViT, OFA) has shown that neural networks, especially transformer-based models, can leverage the deep fusion of information from multiple views to improve their performance, an aspect that has not been fully explored in the field of multi-modality few-shot learning.} \jh{To enhance the interaction between vision and language}{To this end}, we design \textbf{D}eeply coupled \textbf{C}ross-modal \textbf{P}rompt learning (DCP) \jh{}{enhancing the language-vision interaction}. Specifically, DCP is built based on CLIP, with additional text and visual prompts across multiple layers. 
% Different from previous methods with deep prompt tuning~\cite{}, DCP only initializes the first layer of visual and text prompt with random vectors. The following prompts are generated by \textbf{C}ross-\textbf{M}odal \textbf{P}rompt \textbf{A}ttention (CMPA) \jh{}{module}, which combines the prompts from the previous layer of two modalities. CMPA brings stronger connection from two aspects \jh{}{, that is, \emph{Breadth} and \emph{Depth}}. 1) \jh{}{\emph{Breadth} means that} CMPA strengthens the correlation of the prompts among different layers. 2) \jh{}{Depth suggests that} CMPA \jh{enhances the interaction}{implements a deep fusion of information} between visual and language modalities. \jhcomment{}{it is better to clarify the relationship between DCP and CMPA somewhere, from my perpective, I can inferred from the paper that CMPA is a module of DCP, but it is better to mention this explicitly} DCP with CMPA actually combines the advantages of single branch and dual-branch multi-modal pre-training methods, which can decrease the discrepancy between visual and text \jh{}{knowledge} without adding too much trainable parameters.

% % CMPA是一种怎样的方法，有哪些优势
% We verify our method by conducting experiments on 11 datasets under few-shot setting following CoOp. The 11 datasets covers different image classification tasks including generic objects, scenes, actions and fine-grained categories \jh{}{to form a comprehensive benchmark}. We compare our method with visual prompt tuning, text prompt tuning and multi-modal prompt tuning methods. The results demonstrate the effectiveness of our method. Further, ... \jhcomment{}{maybe reword this paragraph as contributions "To conclude, the contributions of this work are as follows: ...."}

==> method.tex <==
\section{Method}
In this section, we first introduce the preliminaries, including CLIP~\cite{DBLP:conf/icml/RadfordKHRGASAM21}, CoOp~\cite{DBLP:journals/ijcv/ZhouYLL22} and VPT~\cite{DBLP:conf/eccv/JiaTCCBHL22}. CLIP is a vision-language pre-trained method which is the backbone of our approach. CoOp is a text prompt tuning method based on CLIP and VPT is a visual prompt tuning method based on ViT~\cite{DBLP:conf/iclr/DosovitskiyB0WZ21}. Then, we present the details of our deeply coupled prompt learning (DCP), which can enhance the interaction between vision and text with cross-modal prompt attention module (CMPA). CMPA can connect the prompts cross layers and domains.

\begin{figure*}[tp]
	\centering
	\includegraphics[width=\textwidth]{figs/pipeline.pdf}
	\caption{The pipeline of deeply coupled prompt learning.}
	\label{fig:pipeline}
\end{figure*}

% 原始CLIP
\subsection{Preliminaries}
\paragraph{CLIP}
is a dual-encoder pre-trained model which consists of a text encoder and an image encoder. The text and image are independently encoded by the corresponding encoder, then projected to the same embedding space by a projection layer. Specifically, the backbone of the image encoder is ResNet~\cite{DBLP:conf/cvpr/HeZRS16} (d=256) or ViT (d=512), which can map the high-dimension image into a low-dimension embedding.  The text encoder is built based on the decoder of Transformer~\cite{DBLP:conf/nips/VaswaniSPUJGKP17}, which is also known as GPT~\cite{DBLP:conf/nips/BrownMRSKDNSSAA20}, to generate a vectorized representation for a sequence of words. 
% \jhcomment{}{In NLP, the vanilla transformer consists of encoder and decoder, scholars find out encoder-only or decoder-only can also works fine, such as encoder-only model BERT and decoder-only model GPT-3, it is better to examine whether there are any other confused use of encoder, decoder, transformers in the paper.}
The model use a contrastive loss to align the two modalities during training stage.  
The training target is to maximize the cosine similarity for the match image-text pairs and minimize the unmatched ones.

In zero-shot image recognition, the image encoder of CLIP encodes the image into a feature representation $x$. The input text is usually in the form of ``a photo of a \{class\}.'' (\emph{discrete prompt}), where the ``\{class\}'' token is the name of each category. For each dataset containing K categories, a set of text encoders $\{w_i\}_{i=1}^K$ are generated by the text encoder. The prediction probability is computed as
\begin{equation}
p(y \mid \boldsymbol{x})=\frac{\exp \left(\operatorname{cos}\left(\boldsymbol{x}, \boldsymbol{w}_y\right) / \tau\right)}{\sum_{i=1}^K \exp \left(\operatorname{cos}\left(\boldsymbol{x}, \boldsymbol{w}_i\right) / \tau\right)},
\end{equation}
where $\tau$ is a temperature parameter.


% text prompt
\paragraph{CoOp} adapts CLIP to downstream tasks with prompt tuning. Specifically, CoOp tries to learn prompt embedding \emph{(continuous prompt)} during few-shot training to avoid manual prompts. The prompt fed in the text encoder is designed as $t=[V]_1[V]_2...[V]_M[CLASS]$, where $[V]_m \ (m \in \{1,...,M\})$ is initialized with the same dimension as word embeddings. The parameters of the CLIP model is fixed while the prompt is trainable. The prediction probability of CoOp is
\begin{equation}
p(y \mid \boldsymbol{x})=\frac{\exp \left(\operatorname{cos}\left(\boldsymbol{x}, g(\boldsymbol{t}_y\right)) / \tau\right)}{\sum_{i=1}^K \exp \left(\operatorname{cos}\left(\boldsymbol{x}, g(\boldsymbol{t}_i\right)) / \tau\right)},
\end{equation}
where $g(\cdot)$ denotes the text encoder.



% visual prompt
\paragraph{VPT} is an efficient and effective way to adapt large-scale Transformer models in vision with only a small amount of trainable parameters. The backbone of VPT is ViT, which is the same as the image encoder of CLIP. There are two variants of VPT: VPT-Shallow and VPT-Deep. VPT-Shallow only insert prompts into the first layer of the Transformer. The visual prompt can be defined as $p=[P]_1[P]_2...[P]_N$, where $[P]_n \ (n \in \{1,...,N\})$ keeps the same dimension as the image embedding. The input of VPT-shallow is $[x_{cls}, p, x]$, where $x_{cls}$ is the classification token $[CLS]$. VPT-Deep introduces visual prompts at every Transformer layer. The deep VPT can be formulated as
\begin{equation}
\begin{aligned}
{\left[\mathbf{x}_{cls}^i, \ldots, \mathbf{x}^i\right] } & =L^i\left(\left[\mathbf{x}_{cls}^{i-1}, \mathbf{p}^{i-1}, \mathbf{x}^{i-1}\right]\right) \\
i &=1,2, ..., N \\
\mathbf{y} & =\operatorname{Head}\left(\mathbf{x}_{cls}^N\right),
\end{aligned}
\end{equation}
where $N$ denotes the number of Transformer layers and $Head$ is the classification head. Only the prompts and classification head is learning during training. VPT achieves impressive performance on 24 downstream recognition tasks.

% \jhcomment{}{I don't see any connections between CoOp and VPT with our work. It is better to explict mention this, or just remove the corresponding paragraphs.}

% cross modal prompt 
\subsection{Cross-modal Prompt Attention}
Inspired by the success of visual and text prompt leaning, recent studies start multi-modal prompt learning~\cite{DBLP:journals/corr/abs-2210-07225,DBLP:journals/corr/abs-2210-03117}. These methods update the visual and text prompt simultaneously to achieve balance in the learning of visual and text embedding. Although the visual and text embedding are adapted to the few-shot data, the interaction between visual and text is still insufficient. Hence we propose deeply coupled cross-modal prompt learning (DCP), which can enhance the communication between prompts across different layers and modals. The essential module of DCP is cross-modal prompt attention, which fuses visual and text with multi-head cross-modal attention. Figure~\ref{fig:pipeline} depicts the pipeline of DCP and the detailed structure of cross-modal prompt attention (CMPA).

Our method follows the implementation of CLIP, which is also a dual-encoder model. Differently, we add prompts to every branch, and enable information fusion between vision and language during training through CMPA. Specifically, CMPA is a multi-head attention with visual and text prompts as inputs. 
The language prompts of the first layer is initialized with the pre-trained CLIP word embeddings of the template 'a photo of a <class>', it is better to be consistent on the words used., while the visual prompts inserted to the first layer are randomly initialized from a normal distribution. 
Then, the prompts of next layer are generated by CMPA based on the prompts from the previous layer. CMPA can be formulated as 
\begin{equation}
\begin{align}
\text P_t^{l+1}&=\operatorname{softmax}\left(\frac{P_v^l (P_t^l)^T}{\sqrt{d_k}}\right) P_t^l \\
\text P_v^{l+1}&=\operatorname{softmax}\left(\frac{P_t^l (P_v^l)^T}{\sqrt{d_k}}\right) Pv^l \\
l&=1, 2, ..., N-1 ,
\end{align} 
\end{equation}
where $P_t^l$ and $P_v^l$ denotes the text prompt and visual prompt the the $l$ layer of each encoder, respectively. $N$ is the depth of CMPA, which is smaller than the length of text and visual encoder. $d_k$ is the dimension of keys.

Different from previous methods, only the prompts from the first layer are randomly generated. The following prompts depends on the prompts from both visual and language modal. CMPA enable information communication between vision and text through corresponding prompts. Totally, CMPA brings stronger feature fusion from two aspect: layers and modals. Noting that the CMPA share parameters from different layers, the additional trainable parameters is only in a small amount.


==> related.tex <==
\section{Related Work}

\subsection{Vision-language Pre-trained Models}
The advent of Transformer~\cite{DBLP:conf/nips/VaswaniSPUJGKP17} has accelerated the development of large-scale pre-training.
The application of Transformer in the multi-modal is divided into two schools of thought: one is the single-stream model, in which language and vision information are fused at the beginning and fed directly into the encoder together; the other is the dual-stream model, in which language and vision information first pass through two separate encoder modules at the beginning, and then the different modal information is fused through the cross Transformer.

At the outset, basic architecture of some contemporaneous work is BERT. The images are detected with Faster-RCNN~\cite{DBLP:conf/nips/RenHGS15} for region features, and these image region features are fed into BERT along with text information to align the text and image information. Following the same process as BERT, these methods first pre-train and then fine-tune on the corresponding tasks. 
Single-stream networks~\cite{DBLP:journals/corr/abs-1908-03557,DBLP:conf/emnlp/AlbertiLCR19,DBLP:journals/corr/abs-1909-11740,DBLP:conf/aaai/LiDFGJ20,DBLP:conf/iclr/SuZCLLWD20,DBLP:conf/aaai/ZhouPZHCG20,DBLP:journals/corr/abs-2001-07966,DBLP:conf/cvpr/LuGRPL20} fuse information from different modalities directly through an encoder.
The dual-stream models~\cite{DBLP:conf/nips/LuBPL19,DBLP:conf/emnlp/TanB19} integrate different modal information through cross modal transformer. 
% Empirically single-stream networks are more sufficient for information fusion, while dual-stream networks can be more efficient for training due to less training parameters. \jhcomment{}{I think remove this statement since it bring no information regarding our work.}

Recent cross-modal large-scale pre-training models have made greater breakthroughs in training data magnitude and tasks by devising various model architectures and training objectives, and have achieved impressive performance in many downstream tasks. CLIP~\cite{DBLP:conf/icml/RadfordKHRGASAM21} and ALIGN~\cite{DBLP:conf/icml/JiaYXCPPLSLD21} got remarkable zero-shot results after pre-trained on millions or billions of (image, text) pairs collected from the internet. Coca~\cite{DBLP:journals/corr/abs-2205-01917} combined the advantages of the contrast learning method~\cite{DBLP:conf/icml/RadfordKHRGASAM21} and the generative model SiMVLM~\cite{DBLP:conf/iclr/WangYYDT022} by adding caption loss to the contrast loss of CLIP.
OFA~\cite{DBLP:conf/icml/WangYMLBLMZZY22}, Unified-IO~\cite{DBLP:journals/corr/abs-2206-08916} and Florence~\cite{DBLP:journals/corr/abs-2111-11432} unified vision, language and multi-modal tasked  by pre-training on both cross-modal and uni-modal data. These methods have achieved state-fo-the-art results in many downstream tasks.
Some methods are dedicated to improve the performance of certain specific tasks.
UniTAB~\cite{DBLP:conf/eccv/YangGW000LW22} focused on grounded vision-language tasks such as grounded captioning and visual grounding. GLIP~\cite{DBLP:conf/cvpr/LiZZYLZWYZHCG22} unified object detection and phrase grounding for pre-training.
Pre-training models have opened up a situation where deep learning models scale and perform in tandem, becoming a revolutionary breakthrough in artificial intelligence and deep learning.

\subsection{Prompt Learning}
For a long time, first pre-training then fine-tuning was the dominant approach to apply large foundation models to downstream tasks. However, fine-tuning for large models is inefficient and may cause catastrophic forgetting~\cite{DBLP:journals/corr/KirkpatrickPRVD16}. Prompt learning is proposed to address the above problems. The prompt is usually a series of trainable parameters inserted into the input. 
The success of prompt learning in NLP~\cite{DBLP:conf/emnlp/LesterAC21} has inspired its application in other modalities. 
VPT~\cite{DBLP:conf/eccv/JiaTCCBHL22} is a typical successful application of prompt learning on computer vision. Prompt learning has generated more attention and made great progress in cross-modal learning.

SoftCPT~\cite{DBLP:journals/corr/abs-2208-13474} and CPL~\cite{DBLP:journals/corr/abs-2210-10362} applied prompt tuning to different vision and language tasks and outperformed single-task prompt tuning method.
CoOp~\cite{DBLP:journals/ijcv/ZhouYLL22}, ProDA~\cite{DBLP:conf/cvpr/LuLZL022} and UPT~\cite{DBLP:journals/corr/abs-2210-07225} adapted prompt learning to traditional few-shot visual recognition with CLIP as backbone. CoCoOp~\cite{DBLP:conf/cvpr/ZhouYL022}, ProGrad~\cite{DBLP:journals/corr/abs-2205-14865} and MaPLe~\cite{DBLP:journals/corr/abs-2210-03117} improved the classification performance of pre-trained models on novel categories by prompt learning. 
Different from previous method, our approach brings stronger connection between modalities and layers with proposed cross-modal prompt attention. The stronger interaction between vision and language enable the our method get state-of-the-art performance in few-shot learning.

% Our approach concentrates on traditional few-shot image classification by cross-modal prompt learning mechanisms to enhance the interaction between different modalities. 
% \jhcomment{}{Related work is a good chance to re-emphasize the gap in the literature and the distinct features of our method to close the gap.}
% Visual Prompt Tuning for Few-Shot Text Classification
% Prompt Tuning with Soft Context Sharing for Vision-Language Models
% CPL: Counterfactual Prompt Learning for Vision and Language Models
% Prompting through Prototype: A Prototype-based Prompt Learning on Pretrained Vision-Language Models
% Unified Vision and Language Prompt Learning
% Neural Prompt Search
% Prompt-aligned Gradient for Prompt Tuning
% Prompt Distribution Learning
% MaPLe: Multi-modal Prompt Learning
% Unsupervised Prompt Learning for Vision-Language Models
% Variational prompt tuning improves generalization of vision-language models
% Modular and Parameter-Efficient Multimodal Fusion with Prompting
% Conditional prompt learning for vision-language models


% Prompt Learning with Optimal Transport for Vision-Language Models
% Fine-grained Retrieval Prompt Tuning
% Learning to Prompt for Open-Vocabulary Object Detection with Vision-Language Model
% Prompt-matched semantic segmentation
% CLIP also Understands Text: Prompting CLIP for Phrase Understanding
% Vqgan-clip: Open domain image generation and editing with natural language guidance

